RIS Deployment Optimization with Iterative Detection and Decoding in Multiuser Multiple-Antenna Systems

This work investigates a Reconfigurable Intelligent Surface (RIS)-assisted uplink system employing iterative detection and decoding (IDD) techniques. We analyze the impact of tuning system parameter tuning for several deployment configurations, including the number of users, access point (AP) antennas, and RIS elements on the IDD performance. Analytical results for both active and passive RIS in a single-input single-output (SISO) scenario demonstrate how deployment choices affect system performance. Numerical simulations confirm the robustness of the RIS-assisted IDD system to variations in these parameters, showing performance gains in certain configurations. Moreover, the findings indicate that the insights derived from SISO analysis extend to multiuser MIMO IDD systems.

==> Figure2/Fig_active.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
%width=1.946in,
width=1.946in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=49.9,
xmax=400,
xtick={ 50, 100, 200, 300, 400},
xlabel style={font=\color{white!15!black}},
xlabel={$d$},
ymin=0,
ymax=70,
ylabel style={font=\color{white!15!black}},
ylabel={Sum-Rate bits/Hz},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt, mark=square, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
50	63.2472887234686\\
100	47.5567913838549\\
150	36.4439427683328\\
200	29.0174994683515\\
250	24.0073875282763\\
300	20.3050271247923\\
350	17.5686596862859\\
400	14.0260902458033\\
};
\addlegendentry{MMSE A-RIS}

\addplot [color=mycolor2, line width=2.0pt, mark=square, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
50	60.546564070214\\
100	38.0201234543959\\
150	26.7793276068054\\
200	20.192229947937\\
250	16.0899464413146\\
300	13.1993727721778\\
350	11.1476459393933\\
400	8.75684178321243\\
};
\addlegendentry{$\text{IDD MMSE A-RIS }\tau\text{ = 1}$}

\addplot [color=mycolor3, line width=2.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
50	60.5463903563409\\
100	38.0246476944094\\
150	26.7879265743861\\
200	22.0035972884364\\
250	17.5790806103244\\
300	14.0701046176964\\
350	11.7444439574233\\
400	9.07003616650306\\
};
\addlegendentry{$\text{IDD MMSE A-RIS }\tau\text{ = 3}$}

\end{axis}

\begin{axis}[%
width=1.946in,
height=3.566in,
at={(3.327in,0.481in)},
scale only axis,
xmin=50,
xmax=400,
xtick={ 50, 100, 200, 300, 400},
xlabel style={font=\color{white!15!black}},
xlabel={$d$},
ymode=log,
ymin=1e-05,
ymax=1,
ytick={ 1e-05, 0.0001,  0.001,   0.01,    0.1,      1},
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BER},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, line width=2.0pt, mark=square, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
50	2.2e-07\\
100	0.000110677083333\\
150	0.00410205078125\\
200	0.019424153645833\\
250	0.042584635416667\\
300	0.068733723958333\\
350	0.091780598958333\\
400	0.134602864583333\\
};
\addplot [color=mycolor2, line width=2.0pt, mark=square, mark options={solid, mycolor2}, forget plot]
  table[row sep=crcr]{%
50	0\\
100	0\\
150	9.619140625e-06\\
200	0.00967285156249999\\
250	0.078095703125\\
300	0.137652994791667\\
350	0.170732421875\\
400	0.208929036458333\\
};
\addplot [color=mycolor3, line width=2.0pt, mark=square, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
50	0\\
100	0\\
150	4.8828125e-08\\
200	0.001515625\\
250	0.0596907552083333\\
300	0.135026041666667\\
350	0.171236979166667\\
400	0.212454427083333\\
};
\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
